Robust Hierarchical MPC for Handling Long Horizon Demand Forecast Uncertainty with Application to Automotive Thermal Management

This paper presents a robust hierarchical MPC (H-MPC) for dynamic systems with slow states subject to demand forecast uncertainty. The H-MPC has two layers: (i) the scheduling MPC at the upper layer with a relatively long prediction/planning horizon and slow update rate, and (ii) the piloting MPC at the lower layer over a shorter prediction horizon with a faster update rate. The scheduling layer MPC calculates the optimal slow states, which will be tracked by the piloting MPC, while enforcing the system constraints according to a long-range and approximate prediction of the future demand/load, e.g., traction power demand for driving a vehicle. In this paper, to enhance the H-MPC robustness against the long-term demand forecast uncertainty, we propose to use the high-quality preview information enabled by the connectivity technology over the short horizon to modify the planned trajectories via a constraint tightening approach at the scheduling layer. Simulation results are presented for a simplified vehicle model to confirm the effectiveness of the proposed robust H-MPC framework in handling demand forecast uncertainty.

==> CDC_TwoLayerMPC_BTM_CAVs <==
\begin{thebibliography}{10}

\bibitem{medagoda2014multiple}
E.D.M. Medagoda and P.W. Gibbens.
\newblock {Multiple Horizon Model Predictive Flight Control}.
\newblock {\em Journal of Guidance, Control, and Dynamics}, 37(3):946--951,
  2014.

\bibitem{clarke2018hierarchical}
W.C. Clarke, C.~Manzie, and M.J. Brear.
\newblock {Hierarchical Economic MPC for Systems with Storage States}.
\newblock {\em Automatica}, 94:138--150, 2018.

\bibitem{AminiACC19}
M.R. Amini, X.~Gong, H.~Wang, Y.~Feng, I.~Kolmanovsky, and J.~Sun.
\newblock {Sequential Optimization of Speed, Thermal Load, and Power Split in
  Connected HEVs}.
\newblock In {\em ACC}, 2019.
\newblock {Philadelphia, PA, USA}.

\bibitem{AminiCDC18}
M.R. Amini, I.~Kolmanovsky, and J.~Sun.
\newblock {Two-Layer Model Predictive Battery Thermal and Energy Management
  Optimization for Connected and Automated Electric Vehicles}.
\newblock In {\em 57th IEEE CDC}, 2018.
\newblock {Miami Beach, FL, USA}.

\bibitem{Amini_TCST_2019}
M.R. Amini, H.~Wang, X.~Gong, D.~Liao-McPherson, I.~Kolmanovsky, and J.~Sun.
\newblock {Cabin and Battery Thermal Management of Connected and Automated HEVs
  for Improved Energy Efficiency Using Hierarchical Model Predictive Control}.
\newblock {\em IEEE Transactions on Control Systems Technology}, 2019.

\bibitem{koeln2018robust}
J.P. Koeln and A.G. Alleyne.
\newblock {Robust Hierarchical Model Predictive Control of Graph-Based Power
  Flow Systems}.
\newblock {\em Automatica}, 96:127--133, 2018.

\bibitem{koeln2019hierarchical}
J.~Koeln, H.~Pangborn, M.~Williams, M.~Kawamura, and A.~Alleyne.
\newblock {Hierarchical Control of Aircraft Electro-Thermal Systems}.
\newblock {\em IEEE Transactions on Control Systems Technology}, 2019.

\bibitem{barcelliy2010hierarchical}
D.~Barcelliy, A.~Bemporad, and G.~Ripaccioliy.
\newblock {Hierarchical Multi-Rate Control Design for Constrained Linear
  Systems}.
\newblock In {\em 49th CDC}, 2010.
\newblock Atlanta, GA, USA.

\bibitem{scattolini2007hierarchical}
R.~Scattolini and P.~Colaneri.
\newblock {Hierarchical Model Predictive Control}.
\newblock In {\em 46th IEEE CDC}, 2007.
\newblock {New Orleans, LA, USA}.

\bibitem{scattolini2009architectures}
R.~Scattolini.
\newblock {Architectures for Distributed and Hierarchical Model Predictive
  Control--A Review}.
\newblock {\em Process Control}, 19(5):723--731, 2009.

\bibitem{picasso2010mpc}
B.~Picasso, D.~De~Vito, R.~Scattolini, and P.~Colaneri.
\newblock {An MPC Approach to the Design of Two-Layer Hierarchical Control
  Systems}.
\newblock {\em Automatica}, 46(5):823--831, 2010.

\bibitem{Zhen2018Traj}
Z.~Yang, Y.~Feng, X.~Gong, D.~Zhao, and J.~Sun.
\newblock {Eco-trajectory Planning with Consideration of Queue Along Congested
  Corridor for Hybrid Electric Vehicles}.
\newblock In {\em TRB}, 2019.
\newblock {Washington, D.C., USA}.

\bibitem{koeln2018two}
J.P. Koeln and A.G. Alleyne.
\newblock {Two-Level Hierarchical Mission-Based Model Predictive Control}.
\newblock In {\em ACC}, 2018.
\newblock {Milwaukee, WI, USA}.

\bibitem{lofberg2004yalmip}
J.~Lofberg.
\newblock {YALMIP: A Toolbox for Modeling and Optimization in MATLAB}.
\newblock In {\em IEEE CACSD}, 2004.
\newblock {New Orleans, LA, USA}.

\bibitem{wachter2006implementation}
A.~W{\"a}chter and L.~Biegler.
\newblock {On the Implementation of an Interior-Point Filter Line-Search
  Algorithm for Large-Scale Nonlinear Programming}.
\newblock {\em Mathematical Programming}, 106(1):25--57, 2006.

\end{thebibliography}

